Combining Magnetic and Electric Sails for Interstellar Deceleration

The main benefit of an interstellar mission is to carry out in-situ measurements within a target star system. To allow for extended in-situ measurements, the spacecraft needs to be decelerated. One of the currently most promising technologies for deceleration is the magnetic sail which uses the deflection of interstellar matter via a magnetic field to decelerate the spacecraft. However, while the magnetic sail is very efficient at high velocities, its performance decreases with lower speeds. This leads to deceleration durations of several decades depending on the spacecraft mass. Within the context of Project Dragonfly, initiated by the Initiative of Interstellar Studies (i4is), this paper proposes a novel concept for decelerating a spacecraft on an interstellar mission by combining a magnetic sail with an electric sail. Combining the sails compensates for each technologys shortcomings: A magnetic sail is more effective at higher velocities than the electric sail and vice versa. It is demonstrated that using both sails sequentially outperforms using only the magnetic or electric sail for various mission scenarios and velocity ranges, at a constant total spacecraft mass. For example, for decelerating from 5% c, to interplanetary velocities, a spacecraft with both sails needs about 29 years, whereas the electric sail alone would take 35 years and the magnetic sail about 40 years with a total spacecraft mass of 8250 kg. Furthermore, it is assessed how the combined deceleration system affects the optimal overall mission architecture for different spacecraft masses and cruising speeds. Future work would investigate how operating both systems in parallel instead of sequentially would affect its performance. Moreover, uncertainties in the density of interstellar matter and sail properties need to be explored.

==> nomenclature.tex <==
\section*{Nomenclature}
Abbreviations:\\
%\noindent{Abbreviations}
\vbox{\noindent\setlength{\tabcolsep}{0mm}%
\begin{tabular}{p{25mm}cl} %

\hfil Msail \hfil & :\hspace{4mm} & Magnetic Sail \\
\hfil Esail \hfil & :\hspace{4mm} & Electric Sail \\
\hfil i4is \hfil & :\hspace{4mm} & Institute for Interstellar Studies \\
\hfil AU \hfil & :\hspace{4mm} & Astronomical unit \\
\hfil $M_{\odot}$ \hfil & :\hspace{4mm} & Solar mass \\
\hfil MSL \hfil & :\hspace{4mm} & Mars Science Laboratory 
\end{tabular}}\\


Symbols: \\
%\noindent{Symbols}
%\vbox{\noindent\setlength{\tabcolsep}{0mm}%
\resizebox{\linewidth}{!}{
\begin{tabular}{p{25mm}cl} %
\hfil$v$\hfil & :\hspace{4mm} & velocity $\mathrm{(m/s)}$\\
\hfil$F$\hfil & :\hspace{4mm} & force $\mathrm{(N)}$\\
\hfil$m_p$\hfil & :\hspace{4mm} & proton mass $\mathrm{(kg)}$\\
\hfil$n_o$\hfil & :\hspace{4mm} & interstellar proton density $\mathrm{(m^{-3})}$\\
\hfil$\mu$\hfil & :\hspace{4mm} & free space permeability $\mathrm{(N/A^2)}$\\
\hfil$I$\hfil & :\hspace{4mm} & magnetic sail current $\mathrm{(A)}$\\
\hfil$R$\hfil & :\hspace{4mm} & magnetic sail radius $\mathrm{(km)}$\\
\hfil$j_{max}$\hfil & :\hspace{4mm} & critical current density $\mathrm{(A/m^2)}$\\
\hfil$\rho_{Msail}$\hfil & :\hspace{4mm} & magnetic sail mass density $\mathrm{(kg/m^3)}$\\
\hfil$m_{shield}$\hfil & :\hspace{4mm} & magnetic sail shield mass $\mathrm{(kg)}$\\
\hfil$A_{ion}$\hfil & :\hspace{4mm} & coil cross sectional area $\mathrm{(m^2)}$\\
\hfil$\Delta H$\hfil & :\hspace{4mm} & vaporization enthalpy $\mathrm{(J/kg)}$\\
\hfil$c$\hfil & :\hspace{4mm} & speed of light $\mathrm{(m/s)}$\\
\hfil$\beta$\hfil & :\hspace{4mm} & ratio of velocity to speed of light $\mathrm{(-)}$\\
\hfil$N$\hfil & :\hspace{4mm} & number of electric sail tethers $\mathrm{(-)}$\\
\hfil$L$\hfil & :\hspace{4mm} & length of electric sail tethers $\mathrm{(km)}$\\
\hfil$r_o$\hfil & :\hspace{4mm} & double Debye length $\mathrm{(m)}$\\
\hfil$\lambda_D$\hfil & :\hspace{4mm} & Debye length $\mathrm{(m)}$\\
\hfil$e$\hfil & :\hspace{4mm} & electron charge $\mathrm{(C)}$\\
\hfil$V_o$\hfil & :\hspace{4mm} & electric sail voltage $\mathrm{(V)}$\\
\hfil$r_w$\hfil & :\hspace{4mm} & electric sail wire radius $\mathrm{(\mu m)}$\\
\hfil$\epsilon_o$\hfil & :\hspace{4mm} & electric permittivity of vacuum $\mathrm{(F/m)}$\\
\hfil$k_b$\hfil & :\hspace{4mm} & Boltzmann constant $\mathrm{(J/K)}$\\
\hfil$T_e$\hfil & :\hspace{4mm} & interstellar plasma temperature $\mathrm{(K)}$\\
\hfil$P$\hfil & :\hspace{4mm} & electric sail power $\mathrm{(W)}$\\
\hfil$a$\hfil & :\hspace{4mm} & acceleration $\mathrm{(m/s)}$\\
\hfil$\Delta v$\hfil & :\hspace{4mm} & velocity change $\mathrm{(km/s)}$\\
\hfil$\Delta v_{Msail}$\hfil & :\hspace{4mm} & velocity change with magnetic sail $\mathrm{(km/s)}$\\
\hfil$\Delta v_{Esail}$\hfil & :\hspace{4mm} & velocity change with electric sail $\mathrm{(km/s)}$\\
\hfil$m_{s/c}$\hfil & :\hspace{4mm} & spacecraft mass $\mathrm{(kg)}$\\
\hfil$m_{Msail}$\hfil & :\hspace{4mm} & magnetic sail mass $\mathrm{(kg)}$\\
\hfil$m_{Esail}$\hfil & :\hspace{4mm} & electric sail mass $\mathrm{(kg)}$\\
\hfil$v_{target}$\hfil & :\hspace{4mm} & target spacecraft velocity $\mathrm{(km/s)}$\\
\hfil$v_{cruise}$\hfil & :\hspace{4mm} & cruising velocity $\mathrm{(km/s)}$\\
\hfil$T_{decel}$\hfil & :\hspace{4mm} & deceleration duration (years)
\end{tabular}
}


